Combining Public and Private Data

Differential privacy is widely adopted to provide provable privacy guarantees in data analysis. We consider the problem of combining public and private data (and, more generally, data with heterogeneous privacy needs) for estimating aggregate statistics. We introduce a mixed estimator of the mean optimized to minimize the variance. We argue that our mechanism is preferable to techniques that preserve the privacy of individuals by subsampling data proportionally to the privacy needs of users. Similarly, we present a mixed median estimator based on the exponential mechanism. We compare our mechanisms to the methods proposed in Jorgensen et al. [2015]. Our experiments provide empirical evidence that our mechanisms often outperform the baseline methods.

==> alexnotes.tex <==
\subsection*{Alex's comments, 06/25}
\\
\\
Why subsampling shouldn't help:
\\
\\
suppose for a moment that there are no public points. then we are just computing the DP mean of a private sample. alpha doesn't do anything interesting here, so the only question is whether we can get an advantage by subsampling. (intuitively, this already seems unlikely.)
\\
\\
suppose we have m points and we subsample them by a factor of $p, 0 < p <= 1$. we can expect to have about mp points in our subsample, and we will then be able to use noise with privacy parameter epsilon / p. (this is not exactly true -- the parameter is going to be slightly less generous than that -- but it's close for small enough epsilon, and i am arguing that subsampling is bad so giving it an advantage should be okay.)
\\
\\
so the variance of the mean with Laplace noise would be something like:

$$\frac{mp \sigma^2 + 2 r^2 p^2 / \epsilon^2}{(mp)^2} = \frac{\sigma^2}{mp} + \frac{2 r^2 / \epsilon^2}{m^2}$$

clearly, this is minimized by setting p = 1. The noise term is not affected by p at all, and of course the sample mean term is going to be minimized when we have the most points. so, as expected, there should be no benefit to subsampling when just taking a straight private mean.
\\
\\
now suppose we have n public points, which will be kept regardless of p. under PDP, we are going to compute something like:
\\
\\
$$\frac{\sum_{pub} + \sum_{priv} + \nu(\epsilon/p)}{(n + mp)}$$
\\
\\
We can express this as a convex combination of the public sample mean and the private subsample mean:
\\
\\
$$
= A \cdot \frac{\sum_{pub}}{n}  + (1-A) \cdot \frac{\sum_{priv} + \nu(\epsilon/p)}{mp} 
$$
\\
\\
where $A = n / (n + mp)$.
\\
\\
On the other hand, our method is computing:

$$A \cdot \frac{\sum_{pub}}{n} + (1-A) \cdot \frac{\sum_{priv} + \nu(\epsilon)}{m} $$

where $A = n / (n + m \alpha)$. this is almost the same, except that our second term is a straight private mean, whereas the second term for PDP is a subsampled private mean. and we know from the previous argument that subsampling only increases variance in this situation.

so to summarize, there is no benefit to subsampling when computing a private mean. we can view PDP as taking a weighted combination of the public mean and a subsampled private mean. but the latter, being subsampled, is not optimal -- it can be improved by using the full sample instead, which is exactly what we are doing. another way to look at it is that PDP ties A and p together, whereas we are free to combine the optimal A with the optimal p (which is 1).
\\
\\
NOTE: the actual value that the pdp method can use doesn't need to be as large as $\epsilon / p$, which is an overestimate. Based on this paper \url{http://www.cse.chalmers.se/~dave/papers/sampling2016.pdf}, the actual value it can use is $\ln(1 + (1/p) \cdot (\exp(\epsilon) - 1))$.

==> notation.tex <==
% mathbb

\newcommand{\E}{\mathbb{E}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\ind}{\mathbf{1}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\complexes}{\mathbb{C}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\prob}{\mathbb{P}}

% mathcal

\newcommand{\A}{\mathcal{A}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\K}{\mathcal{K}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\N}{\mathcal{N}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}

% bold

\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\bone}{\boldsymbol{1}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\boldeta}{\boldsymbol{\eta}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\renewcommand{\b}{\boldsymbol{b}}
\renewcommand{\c}{\boldsymbol{c}}
\renewcommand{\d}{\boldsymbol{d}}
\newcommand{\e}{\boldsymbol{e}}
\newcommand{\f}{\boldsymbol{f}}
\newcommand{\g}{\boldsymbol{g}}
\newcommand{\h}{\boldsymbol{h}}
\renewcommand{\r}{\boldsymbol{r}}
\renewcommand{\v}{\boldsymbol{v}}
\renewcommand{\u}{\boldsymbol{u}}
\newcommand{\w}{\boldsymbol{w}}
\newcommand{\p}{\boldsymbol{p}}
\newcommand{\q}{\boldsymbol{q}}
\newcommand{\x}{\boldsymbol{x}}
\newcommand{\y}{\boldsymbol{y}}
\newcommand{\z}{\boldsymbol{z}}
\renewcommand{\a}{\boldsymbol{a}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}

% operators

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\st}{\mathrm{s.t.}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\trace}{\mathrm{trace}}
\newcommand{\adj}{\mathrm{adj}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\eig}{\mathrm{eig}}
\newcommand{\KL}{\mathbf{KL}}
\newcommand{\norm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\sqnorm}[2]{\norm{#1}{#2}^2}
\newcommand{\normnlr}[2]{\|#1\|_{#2}}
\newcommand{\sqnormnlr}[2]{\normnlr{#1}{#2}^2}
\newcommand{\iprod}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\df}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ddf}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\newcommand{\proj}[2]{\mathop{\mathrm{proj}}\nolimits_{#1}(#2)}
\newcommand{\inner}[1]{\left \langle {#1} \right \rangle}
\newcommand{\bigo}{\mathcal{O}}
\newcommand{\abs}[1]{\left |#1\right|}

% other

\newcommand{\hL}{\widehat{L}}
\newcommand{\hC}{\widehat{C}}
\newcommand{\hB}{\widehat{B}}
\newcommand{\hb}{\widehat{\boldsymbol{b}}}
\newcommand{\hc}{\widehat{\boldsymbol{c}}}
\newcommand{\hd}{\widehat{\boldsymbol{d}}}
\newcommand{\bb}{\overline{\boldsymbol{b}}}

% organizational

\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{fact}{Fact}
\newtheorem{lemma}{Lemma}
\newtheorem{problem}{Problem}
\newtheorem{proposition}{Proposition}
\newtheorem{reduction}{Reduction}
\newtheorem{theorem}{Theorem}

==> questions.tex <==
\subsection{Optimality results}
[From \href{https://colab.corp.google.com/drive/199bWBkaNC2ldDzxu9Q7JAZTqoYmCdgbY?resourcekey=0-5qn5cZZxVBk6l0auqcFMkA&usp=sharing}{Colab}] Is there another way of combining public and private data that might be better? Or can we show that weighted sum is optimal in some way? Min variance solution? Our solution is unbiased at least, so is this combo also the min variance estimate? Is sample mean min-variance unbiased estimate?
\\
\cecilia{Parametric case: Lehmann–Scheffé theorem could be useful, provided we have a way to compute sufficient statistic}
\\
(Lehmann-Scheffe theorem). Let $X = X_1, X_2, ..., X_n$ be a random sample from a distribution that has p.d.f (or p.m.f in the discrete case) $f(x:\theta)$, where $\theta \in \Omega$ and $\Omega$ is the parameter space. Suppose that there exists a sufficient and complete statistic $T(X)$. If $\theta$ is estimable, then there is a unique unbiased estimator
of $\theta$ that is of the form $h(T)$ with a Borel function $h$. $h(T)$ is the unique uniformly minimum-variance unbiased estimator of $\theta$
\\
(Note: nonparametric distributions). If $X = X_1, X_2, ..., X_n$ is iid from an unknown population $P$ in a nonparametric family $\mathcal{P}$, then in many cases the vector of order statistics $T = (X_{(1)}, ..., X_{(n)})$ is sufficient and complete for $P \in \mathcal{P}$. Note that an estimator $\phi(X_1, ..., X_n)$ is a function of $T$ if and only if the function $\phi$ is symmetric in its $n$ arguments. Hence if $T$ is sufficient and complete, then a symmetric unbiased estimator of any estimable $\theta$ is the UMVUE. (\url{http://pages.stat.wisc.edu/~doksum/STAT709/n709-29.pdf})


